Detect Fake with Fake: Leveraging Synthetic Data-driven Representation for Synthetic Image Detection

Are general-purpose visual representations acquired solely from synthetic data useful for detecting fake images? In this work, we show the effectiveness of synthetic data-driven representations for synthetic image detection. Upon analysis, we find that vision transformers trained by the latest visual representation learners with synthetic data can effectively distinguish fake from real images without seeing any real images during pre-training. Notably, using SynCLR as the backbone in a state-of-the-art detection method demonstrates a performance improvement of +10.32 mAP and +4.73% accuracy over the widely used CLIP, when tested on previously unseen GAN models. Code is available at https://github.com/cvpaperchallenge/detect-fake-with-fake.

==> contents/relatedwork_memo.tex <==
\section{Related Work}
\subsection{Synthetic Image}
\subsubsection{Deepfake.}
\cYoshi{
Synthetic images come in various types, with Deepfake being a prominent example. Deepfake technology utilizes deep learning to manipulate existing videos and audio, creating fictitious moving images that do not exist in reality. This technique primarily targets the generation of facial images of individuals. Deepfake generation methods are diverse, with face swapping being a representative technique. FaceShifter~\cite{li2019faceshifter} and SimSwap~\cite{chen2020simswap} create Deepfakes by swapping the decoder of the trained GAN between the source and target images. Additionally, StyleSwap~\cite{xu2022styleswap} is a robust, high-quality face-swapping method that maps identity information into the latent space.

Other methods for creating Deepfakes include expression swapping~\cite{thies2016face2face, Pumarola_2018_ECCV, nirkin2019fsgan} and attribute manipulation, which alter visual features like age, gender, and hair without changing an individual’s unique identity~\cite{Choi_2018_CVPR, choi2020stargan}.
While these methods generate Deepfakes based on real data, StyleGAN~\cite{karras2019style} and StyleGAN2~\cite{karras2020analyzing} utilize generative models to create entirely fictitious facial images. Those methods are frequently employed for entertainment, but they are also often used for malicious intent.

\subsubsection{Synthetic Image.}
While Deepfakes primarily target facial images, recent advancements in GANs and DMs have enabled the broad replication of features and patterns found in natural images. Consequently, generating diverse and realistic images beyond the domain of faces has become possible. Notably, Latent Diffusion Models (LDM)~\cite{Rombach_2022_CVPR} apply the diffusion process to the latent space rather than the pixel space, simultaneously improving the quality of synthetic images and reducing computational costs. By utilizing the powerful encoder CLIP:ViT~\cite{dosovitskiy2020image, radford2021learning} and the large-scale dataset LAION-5B~\cite{NEURIPS2022_a1859deb}, it has become possible to generate highly diverse, high-quality, and high-resolution images from text prompts.  Additionally, DALL-E~\cite{ramesh2021zero, ramesh2022hierarchical, openai2023dalle3} uses a Transformer as the encoder for VQ-VAE~\cite{oord2018neural, razavi2019generating} to create high-quality images from text. GigaGAN~\cite{kang2023gigagan}, with one billion parameters and cross-attention, generates images comparable to DMs and self-regressive models. Furthermore, methods such as Imagen~\cite{saharia2022photorealistic} and Midjourney~\cite{midjourney} specialize in generating high-resolution and photorealistic images, particularly excelling in the generation of complex scenes and diverse styles.

\subsection{Synthetic Image Detection}
SID~\cite{schinas2024sidbench} involves binary classification to determine whether the input image or video is generated or real.

\subsubsection{Artifact Detection in Image Editing.}
Methods for SID have been proposed even before the significant advancements in generative models. These methods relied on identifying anomalies such as abnormal reflections~\cite{10.1145/2077341.2077345}, resampling~\cite{popescu2005exposing}, and compression artifacts~\cite{agarwal2017photo} that appear during image editing.

\subsubsection{Neural Network-Based Learning.}
With the widespread adoption of deep learning, methods have been proposed for SID~\cite{frank2020leveraging, marra2018detection, rossler2019faceforensics++, shiohara2022detecting} and identifying artifacts from image editing~\cite{cozzolino2015splicebuster, rao2016deep, wang2019detecting} through neural network-based learning.

\subsubsection{Model Generalization Performance.}
However, detection methods that directly learn the features of synthetic images have been noted to overfit to the trained generative models, failing to generalize to images generated by different models~\cite{cozzolino2018forensictransfer, zhang2019detecting}. To address this overfitting issue, various methods have been proposed to improve generalization performance, including learning features standard to multiple generative methods~\cite{yan2023ucf}, using appropriate pre- and post-processing and data augmentation~\cite{wang2020cnn}, employing adversarial training~\cite{chen2022self}, utilizing distance learning~\cite{luo2023prior}, performing data augmentation in the latent space~\cite{yan2024transcending}, comparing patch images~\cite{zhong2024patchcraft}, and detecting traces of up-sampling~\cite{tan2024rethinking}. Additionally, methods have been proposed that use language models to label images as True or Fake based on captions~\cite{keita2024harnessingpowerlargevision}, input images and prompts into ChatGPT to receive text-based responses for classification~\cite{jia2024can}, formulate model architecture attribution as multi-class classification~\cite{shahid2024generalized}, propose an Unseen Fake class to identify fake images from unknown generators~\cite{rahman2023artifact}, and use the fingerprints of generative models~\cite{song2024manifpt, sinitsa2023deepimagefingerprintlow}.

\subsubsection{Based on a Foundational Model.}
Among these efforts to improve generalization performance, Ojha~\etal ~\cite{ojha2023towards} proposed a method that uses the powerful representations of the base model CLIP:ViT directly as a feature extractor. Subsequently, other advanced methods have been proposed, such as combining features from the shallow layers of CLIP:ViT~\cite{koutlis2024leveraging}, integrating CLIP:ViT with multiple LoRAs~\cite{liu2024mixture}, and aligning CLIP:ViT's feature representations with text prompts~\cite{liu2024forgery}. This study builds on the trend of using feature representations from foundational models for SID. Nguyen~\etal~\cite{nguyen2024exploring} conducted extensive analyses on SID based on foundational models, examining the performance differences due to backbone types and the appropriate range of backbones for fine-tuning. Furthermore, methods such as the fusion of multiple ViT feature representations using MLP-Mixer by Ehab Essa~\cite{ESSA2024128128} and the ensemble of embeddings specialized for each generative model~\cite{azizpour2024e3} have also been proposed. Based on these prior studies, this research aims to improve the generalization performance of detectors by using an ensemble of different foundational models as the backbone.

\subsection{Foundation Model}

A Foundation Model refers to a general-purpose AI model pre-trained on a large-scale dataset. These models are typically built using self-supervised learning and exhibit high versatility across various tasks. Foundation models demonstrate significant adaptability and are widely utilized in various fields, including natural language processing (NLP), image recognition, and speech recognition.

\subsubsection{Transformer and Language Models.}

In 2017, Vaswani~\etal.~\cite{vaswani2017attention} proposed the Transformer architecture, leading to multiple foundation models primarily for language tasks. Devlin~\etal~\cite{devlin2018bert} introduced BERT (Bidirectional Encoder Representations from Transformers), a bidirectional Transformer encoder that achieved state-of-the-art results in NLP tasks. Radford\etal~\cite{radford2018improving} proposed GPT, a powerful model for generative tasks utilizing a unidirectional Transformer decoder. Subsequently, Brown\etal~\cite{brown2020language} demonstrated GPT-3's ability to handle a wide range of NLP tasks with a few task examples. The T5 (Text-To-Text Transfer Transformer)~\cite{raffel2020exploring} model was introduced, treating all NLP tasks as text generation problems. This approach enhanced the efficiency of transfer learning across tasks by processing various NLP tasks in a unified text generation format.

\subsubsection{Vision Transformer and Visual Foundation Models.}

Vision Transformer (ViT)~\cite{dosovitskiy2020image} applied the Transformer architecture to image recognition tasks for the first time, demonstrating high performance without relying on traditional CNNs. This breakthrough led to the emergence of various foundation models. CLIP (Contrastive Language-Image Pre-Training)~\cite{radford2021learning} achieved high performance in visual tasks through pre-training on text-image pairs. DINO (Distillation with NO labels)~\cite{caron2021emerging} is a self-supervised learning method leveraging knowledge distillation to learn feature representations from unlabeled data. An improvement on DINO, DINOv2 (Self-Distillation with No Labels)~\cite{oquab2023dinov2}, extracts high-quality visual features independently of the dataset by combining self-distillation and contrastive learning, achieving superior performance.

Additionally, MERU~\cite{desai2023meru}, which learns image and language representations in hyperbolic space, effectively captures hierarchical data structures compared to traditional Euclidean space. This approach naturally grasps the relationship between images and language, achieving high accuracy, particularly in image caption generation and retrieval.

\subsubsection{Training with Synthetic Images and LLMs.}

While previous methods focused on learning using real images and text data, training with synthetic images and LLMs has become increasingly common. VisualAtom~\cite{takashima2023visual}, specialized in representation learning of visual data, developed a novel approach based on toroidal harmonics to optimize parameters, leveraging the effectiveness of Formula-driven supervised learning (FDSL) during ViT pre-training. This study confirmed the importance of diversity in synthetic images.

Tian~\etal proposed Stablerep~\cite{NEURIPS2023_971f1e59}, which conducts self-supervised learning using text data and image generation models without using any real data. They also introduced SynCLR~\cite{Tian_2024_CVPR}, a method for contrastive learning that employs LLMs and image generation models. Krishnakant Singh~\etal ~\cite{Singh_2024_CVPR} evaluated the robustness of models trained with synthetic data in out-of-distribution (OOD) detection.

\subsubsection{Models Used in This Study.}

This study employs CLIP and DINOv2, foundational models trained solely on real images, as well as StableRep and SynCLR, foundational models trained using synthetic data from synthetic images and LLMs, for SID.}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%以下、メモ
% 生成画像には多様な種類が存在するが，代表例としてDeepfakeが挙げられる．
% Deepfakeは深層学習を使用して既存の映像や音声を操作することで，現実には存在しない架空の動画像を生成する技術のことであり，主として人物の顔画像を生成の対象とするものである．

% Deepfakeの生成手法も多岐にわたるが，代表的な手法として顔交換の手法が挙げられる．
% FaceShifter~\cite{li2019faceshifter}やSimSwap~\cite{chen2020simswap}は，学習したGANのデコーダーをソース画像とターゲット画像間で交換することで，ターゲット画像の表情は変化させずに，ソース画像の顔をターゲット画像の顔に転写することでDeepfakeを作成する．
% また，アイデンティティの情報を潜在空間にマッピングすることでロバストで，高品質なDeepfakeを生成する顔交換の手法として StyleSwap~\cite{xu2022styleswap}がある．

% その他にも，人物の表情やその動きを操作する表情交換によりDeepfakeを生成する手法~\cite{thies2016face2face, Pumarola_2018_ECCV,nirkin2019fsgan }や，個人特有のアイデンティティを変更せずに年齢や性別，髪といった外見の情報を操作する属性操作による手法~\cite{Choi_2018_CVPR,choi2020stargan}も存在する．
% 上記の手法は実データを元にDeepfakeの生成を行うが，StyleGAN~\cite{karras2019style}や StyleGAN2~\cite{karras2020analyzing}は生成モデルを使用して，存在しない架空の人物の顔画像全体を生成する．
% 架空の人物の生成はエンターテイメント目的で多く利用されている一方で，悪意のある用途で使用されるケースも多い．

% Synthetic images come in various types, with Deepfake being a prominent example. Deepfake technology utilizes deep learning to manipulate existing videos and audio, creating fictitious moving images that do not exist in reality. This technique primarily targets the generation of facial images of individuals. Deepfake generation methods are diverse, with face swapping being a representative technique. FaceShifter~\cite{li2019faceshifter} and SimSwap~\cite{chen2020simswap} create Deepfakes by swapping the decoder of the trained GAN between the source and target images, transferring the face from the source image to the target image without altering the target image's expression. Additionally, StyleSwap~\cite{xu2022styleswap} is a robust, high-quality face-swapping method that maps identity information into the latent space.

% Other methods for creating Deepfakes include techniques that manipulate facial expressions and movements, such as expression swapping~\cite{thies2016face2face, Pumarola_2018_ECCV, nirkin2019fsgan}, as well as attribute manipulation methods that alter visual features like age, gender, and hair without changing an individual's unique identity~\cite{Choi_2018_CVPR, choi2020stargan}. While these methods generate Deepfakes based on real data, StyleGAN~\cite{karras2019style} and StyleGAN2~\cite{karras2020analyzing} utilize generative models to create entirely fictitious facial images of non-existent individuals. The generation of fictitious individuals is frequently employed for entertainment purposes, yet it is also often used for malicious intent.

% \subsubsection{Synthetic Image.}
% Deepfakeは主に顔画像を対象とした生成画像であるが，近年はGANやDMの発展により自然画像が持っている特徴やパターンを広く再現することが可能となったため，顔のドメインに縛られない多様な画像を写実的に生成出来るようになった．
% 特にLatent diffusion models (LDM)~\cite{Rombach_2022_CVPR}は従来のピクセル空間における拡散過程ではなく，潜在空間に対して拡散過程を適用することで生成画像の品質の向上と計算コストの削減を同時に実現した． 

% CLIP:ViT~\cite{dosovitskiy2020image,radford2021learning}を使用した強力なエンコーダと大規模データセットであるLAION-5B~\cite{NEURIPS2022_a1859deb}を用いた学習によって，テキストプロンプトから非常に多様な高品質かつ高解像度の画像を生成することを可能とした．
% また，DALL-E~\cite{ramesh2021zero, ramesh2022hierarchical, openai2023dalle3}はVQ-VAE~\cite{oord2018neural, razavi2019generating}のエンコーダとしてTransformerを使用することで，テキストから高品質画像を生成する自己回帰モデルを実現した．
% GigaGAN~\cite{kang2023gigagan}はCross-attentionなどの導入により従来のGANのパラメータ数を10億まで増やし，DMや自己回帰モデルと同水準の高品質画像の生成を可能にした．
% 他にも，高解像度かつ写実的な画像生成に特化しており，特に複雑なシーンや多様なスタイルの画像生成に優れているImagen~\cite{saharia2022photorealistic}やMidjourney~\cite{midjourney}など多様な画像生成手法が提案されている．

% While Deepfakes primarily targets facial images, recent advancements in GANs and DMs have enabled the broad replication of features and patterns found in natural images. Consequently, generating diverse and realistic images beyond the domain of faces has become possible. Notably, Latent Diffusion Models (LDM)~\cite{Rombach_2022_CVPR} apply the diffusion process to the latent space rather than the pixel space, simultaneously improving the quality of synthetic images and reducing computational costs. By utilizing the powerful encoder CLIP:ViT~\cite{dosovitskiy2020image, radford2021learning} and the large-scale dataset LAION-5B~\cite{NEURIPS2022_a1859deb}, it has become possible to generate highly diverse, high-quality, and high-resolution images from text prompts. Additionally, DALL-E~\cite{ramesh2021zero, ramesh2022hierarchical, openai2023dalle3} employs a Transformer as the encoder for VQ-VAE~\cite{oord2018neural, razavi2019generating}, achieving a self-regressive model that generates high-quality images from text. GigaGAN~\cite{kang2023gigagan} has increased the number of parameters in traditional GANs to one billion through the introduction of cross-attention, enabling the generation of high-quality images on par with DMs and self-regressive models. Furthermore, methods such as Imagen~\cite{saharia2022photorealistic} and Midjourney~\cite{midjourney} specialize in generating high-resolution and photorealistic images, particularly excelling in the generation of complex scenes and diverse styles.

% \subsection{Synthetic Image Detection}
% 生成画像検出~\cite{schinas2024sidbench}は入力された画像や動画が生成画像であるか実画像であるかの二値分類を行うタスクである．

% \subsubsection{Artifact base that appears during image editing.}

% 異常な反射: Exposing photo manipulation with inconsistent reflections
% リサンプリング: Exposing digital forgeries by detecting traces of resampling
% 圧縮のアーティファクト: Photo forensics from jpeg dimples. 

% 生成画像検出の手法は生成モデルの飛躍的な発展以前から提案されており，画像編集の際に現れる異常な反射~\cite{10.1145/2077341.2077345}やリサンプリング~\cite{popescu2005exposing}，圧縮のアーティファクト~\cite{agarwal2017photo}などを使用して検出を行っていた．


% \subsubsection{Learning-based using neural networks.}
% <ニューラルネットワークを使用した学習によって生成画像の検出>
% Leveraging frequency analysis for deep fake image recognition
2020
周波数空間では、GAN で生成された画像に簡単に識別できる深刻なアーティファクトが見られることを結果から明らかにしました
CNN

% Detection of gan-generated fake images over social networks
2018
従来の検出器とディープラーニング検出器など、いくつかを比較、調査
圧縮されたデータで最大の高い精度を提供し続けているのはディープラーニング検出器

% FaceForensics++: Learning to detect manipulated facial images.
2019
顔操作検出の自動ベンチマーク（データセット）を提案
データ駆動型の偽造検出器の徹底的な分析 CNN

% Detecting Deepfakes with Self-Blended Images
2023
Efficientnetでデータを学習
学習データの提案

% <ニューラルネットワークを使用した学習によって画像編集のアーティファクトを検出する手法>
% Splicebuster: A new blind image splicing detector
2015
事前情報なしで画像のスプライシングを検出する新しい特徴ベースのアルゴリズムを提案
期待値最大化アルゴリズムと、本物とスプライシングされた部分のセグメンテーションを通じて画像自体によって学習されます

% A deep learning approach to detection of splicing and copy-move forgeries in images
2016
CNNを利用して入力 RGB カラー画像から階層表現を自動的に学習する、ディープラーニング技術に基づく新しい画像偽造検出方法
画像スプライシングおよびコピー移動検出アプリケーション向けに特別に設計

% Detecting photoshopped faces by scripting photoshop
2019
Photoshop 自体のスクリプトによって自動的に生成された偽の画像のみを使用してトレーニングされたモデルを使用して、非常に一般的な Photoshop 操作の 1 つである、人間の顔に適用された画像の歪みを検出する方法を紹介

% 深層学習の普及に従って，ニューラルネットワークを使用した学習によって生成画像の検出~\cite{frank2020leveraging, marra2018detection, rossler2019faceforensics++, shiohara2022detecting}や画像編集のアーティファクトの検出~\cite{cozzolino2015splicebuster, rao2016deep, wang2019detecting}をする手法が提案された．

% \subsubsection{Model generalisation performance.}
% <汎化しないことが指摘された>
% Forensictransfer: Weaklysupervised domain adaptation for forgery detection. 
% Detecting and simulating artifacts in gan fake images. 

% しかしながら，生成された画像の特徴を直接学習する検出手法は，学習した生成モデルに対して過剰適合をしてしまい，異なるモデルを用いて生成された画像の検出には汎化しないことが指摘された~\cite{cozzolino2018forensictransfer, zhang2019detecting}．

% 生成手法に共通する特徴を学習する方法: UCF: Uncovering Common Features for Generalizable Deepfake Detection
2023 33

% Adversarial Trainingを使用する方法: Self-supervised Learning of Adversarial Example: Towards Good Generalizations for Deepfake Detection
2022 164

% 距離学習の使用: Beyond the Prior Forgery Knowledge: Mining Critical Clues for General Face Forgery Detection
2023 15

% 潜在空間でデータ拡張を行う方法: Transcending Forgery Specificity with Latent Space Augmentation for Generalizable Deepfake Detection
2024 4

% パッチ同士の比較: PatchCraft: Exploring Texture Patch for Efficient AI-generated Image Detection
2023 11

% up-samplingの痕跡を検出する方法: Rethinking the Up-Sampling Operations in CNN-based Generative Network for Generalizable Deepfake Detection
2024 9

% この過剰適合への対策として，複数の生成手法に共通する特徴の学習~\cite{yan2023ucf}，適切な事前・事後処理とデータ拡張~\cite{wang2020cnn}, Adversarial Trainingの使用~\cite{chen2022self}，距離学習の使用~\cite{luo2023prior}，潜在空間でのデータ拡張~\cite{yan2024transcending}，パッチ画像同士の比較~\cite{zhong2024patchcraft}，up-samplingの痕跡の検出~\cite{tan2024rethinking}など汎化性能を向上させる様々な手法が提案されてきた．
%  適切な事前・事後処理とデータ拡張:CNN-generated images are surprisingly easy to spot... for now

% その他にも，
言語モデルを使用して、画像のキャプションとしてTrueかFakeかをラベル付けする手法~\cite{keita2024harnessingpowerlargevision}
2024
やChatGPTに画像とプロンプトを入力して、文章でレスポンスを受け取って分類する手法~\cite{jia2024can}，
2024 4
モデルのアーキテクチャの帰属を他クラス分類として定式化した手法~\cite{shahid2024generalized}、
2024
未見の生成器からのフェイク画像を識別するためのUnseen Fakeクラスを提案した手法~\cite{rahman2023artifact}、
2023 10

生成モデルのフィンガープリントを使用した手法がある~\cite{song2024manifpt, sinitsa2023deepimagefingerprintlow}。
ManiFPT: Defining and Analyzing Fingerprints of Generative Models
2024 1
Deep Image Fingerprint: Towards Low Budget Synthetic Image Detection and Model Lineage Analysis
2024 5




% 拡散モデルに固有のパターンとノイズ特性を分析する手法~\cite{wang2023dire}

% \subsubsection{based on a foundational model.}

% このような汎化性能向上の取り組みの中で，Ojhaら~\cite{ojha2023towards}によって基盤モデルであるCLIP:ViTの強力な表現を特徴量抽出器としてそのまま使用する手法が提案され，その後も発展的な手法として，CLIP:ViTの浅い層の特徴を組み合わせて使用する手法~\cite{koutlis2024leveraging}，CLIP:ViTと複数のLoRAを組み合わせる手法~\cite{liu2024mixture}，CLIP:ViTの特徴表現をテキストプロンプトでアラインメントする手法~\cite{liu2024forgery}などが提案された．

% 以下の文章をなおす必要あり

% 本研究はこの基盤モデルの特徴表現を使用した生成画像検出手法の流れを受けたものである。
% Nguyenら~\cite{nguyen2024exploring}は基盤モデルに基づく生成画像検出に関してバックボーンの種類による性能の違いやfinetuneを行う適切なバックボーンの範囲などについて広範な分析を行っている。
% さらに、Ehab Essa~\cite{ESSA2024128128}のMLP-Mixerを使って複数のViTの特徴表現を融合する手法や、各生成モデルに特化した埋め込みをアンサンブルする手法~\cite{azizpour2024e3}も提案されている。
% 本研究ではこれらの先行研究に基づき、異なる基盤モデルのアンサンブルによる組み合わせをバックボーンとして使用することにより、検出器の汎化性能を向上させることを目的としている。


% \subsection{Synthetic Image Detection}
% SID~\cite{schinas2024sidbench} involves binary classification to determine whether the input image or video is generated or real.

% \subsubsection{Artifact Detection in Image Editing.}
% Methods for SID have been proposed even before the significant advancements in generative models. These methods relied on identifying anomalies such as abnormal reflections~\cite{10.1145/2077341.2077345}, resampling~\cite{popescu2005exposing}, and compression artifacts~\cite{agarwal2017photo} that appear during image editing.

% \subsubsection{Neural Network-Based Learning.}
% With the widespread adoption of deep learning, methods have been proposed for SID~\cite{frank2020leveraging, marra2018detection, rossler2019faceforensics++, shiohara2022detecting} and identifying artifacts from image editing~\cite{cozzolino2015splicebuster, rao2016deep, wang2019detecting} through neural network-based learning.

% \subsubsection{Model Generalization Performance.}
% However, detection methods that directly learn the features of synthetic images have been noted to overfit to the trained generative models, failing to generalize to images generated by different models~\cite{cozzolino2018forensictransfer, zhang2019detecting}. To address this overfitting issue, various methods have been proposed to improve generalization performance, including learning features common to multiple generative methods~\cite{yan2023ucf}, using appropriate pre- and post-processing and data augmentation~\cite{wang2020cnn}, employing adversarial training~\cite{chen2022self}, utilizing distance learning~\cite{luo2023prior}, performing data augmentation in the latent space~\cite{yan2024transcending}, comparing patch images~\cite{zhong2024patchcraft}, and detecting traces of up-sampling~\cite{tan2024rethinking}. Additionally, methods have been proposed that use language models to label images as True or Fake based on captions~\cite{keita2024harnessingpowerlargevision}, input images and prompts into ChatGPT to receive text-based responses for classification~\cite{jia2024can}, formulate model architecture attribution as multi-class classification~\cite{shahid2024generalized}, propose an Unseen Fake class to identify fake images from unknown generators~\cite{rahman2023artifact}, and use the fingerprints of generative models~\cite{song2024manifpt, sinitsa2023deepimagefingerprintlow}.

% \subsubsection{Based on a Foundational Model.}
% Among these efforts to improve generalization performance, Ojha~\etal ~\cite{ojha2023towards} proposed a method that uses the powerful representations of the base model CLIP:ViT directly as a feature extractor. Subsequently, other advanced methods have been proposed, such as combining features from the shallow layers of CLIP:ViT~\cite{koutlis2024leveraging}, integrating CLIP:ViT with multiple LoRAs~\cite{liu2024mixture}, and aligning CLIP:ViT's feature representations with text prompts~\cite{liu2024forgery}. This study builds on the trend of using feature representations from foundational models for SID. Nguyen~\etal~\cite{nguyen2024exploring} conducted extensive analyses on SID based on foundational models, examining the performance differences due to backbone types and the appropriate range of backbones for fine-tuning. Furthermore, methods such as the fusion of multiple ViT feature representations using MLP-Mixer by Ehab Essa~\cite{ESSA2024128128} and the ensemble of embeddings specialized for each generative model~\cite{azizpour2024e3} have also been proposed. Based on these prior studies, this research aims to improve the generalization performance of detectors by using an ensemble of different foundational models as the backbone.



%%%%%%%%%
% アンサンブル学習の関連研究
% E3: Ensemble of Expert Embedders for Adapting Synthetic Image Detectors to New Generators Using Limited Data 
% Feature fusion Vision Transformers using MLP-Mixer for enhanced deepfake detection
% Ehab Essa~\cite{ESSA2024128128}のMLP-Mixerを使って複数のViTの特徴表現を融合する手法や、各生成モデルに特化した埋め込みをアンサンブルする手法~\cite{azizpour2024e3}
%%%%%%%%

% \subsection{Foundation Model}

% 基盤モデル（Foundation Model）とは、大規模なデータセットを用いて事前に学習された汎用的なAIモデルのことを指します。これらのモデルは、多くの場合、自己教師あり学習（self-supervised learning）を使用して構築され、多様なタスクに対して高い汎用性を持っています。基盤モデルは、自然言語処理（NLP）、画像認識、音声認識など、様々な分野で広く利用されている。

% Vaswani et al~\cite{vaswani2017attention}らによって2017年にTransformerアーキテクチャが提案され、言語のタスクを中心に複数の基盤モデルが登場した。evlin et al.,らはBERT (Bidirectional Encoder Representations from Transformers)~\cite{devlin2018bert}という双方向のTransformerエンコーダを使用し、NLPタスクで最先端の成果を達成した言語表現モデルを提案し，Radford et alらは一方向のTransformerデコーダを使用し、生成タスクで強力なGPT~\cite{radford2018improving}を提案した。その後、Brown et alによって、 GPT-3~\cite{brown2020language}は少量のタスク例で幅広いNLPタスクをこなせる能力を示した。また、 T5 (Text-To-Text Transfer Transformer)~\cite{raffel2020exploring}と呼ばれる、すべてのNLPタスクをテキスト生成問題として扱うモデルも提案され、様々なNLPタスクを統一されたテキスト生成形式で処理することで、タスク間の転移学習の効率を向上させた。

% 一方で、Alexey Dosovitskiyらによって提案されたVision Transformer(ViT)~\cite{dosovitskiy2020image}は画像認識タスクにおいてTransformerアーキテクチャを初めて適用し、従来のCNNに依存しないアプローチで高い性能を示した。これをきっかけとして、様々な基盤モデルが登場した。CLIP (Contrastive Language-Image Pre-Training)~\cite{radford2021learning}はテキストと画像のペアを用いた事前学習で視覚タスクに高い性能を示した。DINO（Distillation with NO labels）~\cite{caron2021emerging}は、知識蒸留を活用した自己教師あり学習手法であり、ラベルなしデータから特徴表現を学習する。DINOに改良を加えたのが、DINOv2 (Self-Distillation with No Labels)~\cite{oquab2023dinov2}であり、データセットに依存せずに高品質な視覚特徴を抽出し、自己蒸留とコントラスト学習を組み合わせることで、優れた性能を達成している。

% その他にも、 画像と言語の表現を双曲空間で学習したMERU~\cite{desai2023meru}は、従来のユークリッド空間に比べ、階層的なデータ構造を効果的に表現できるため、画像と言語の関連性をより自然に捉え、特に画像キャプション生成や画像検索において高い精度を達成した。 

% これまでの手法では、実画像やテキストデータを使用して学習を行っていたのに対して、生成画像やＬＬＭを使用した学習もおこなわれるようになった。ビジュアルデータの表現学習に特化したVisualAtom~\cite{takashima2023visual}は、ViTの事前学習において、Formula-driven supervised learning（FDSL）が有効であることから、そのパラメータを最適化するために円環調和に基づく新しい手法を開発し、合成画像の多様性が重要であることを確認した。

% Tian et al. は、テキストデータと画像生成モデルを使用して自己教師あり学習を行ったStablerep~\cite{tian2024stablerep}，実データを全く使用せず、LLMと画像生成モデルを使用してコントラスト学習を行う手法のSynCLR~\cite{tian2023learningvisionmodelsrivals}を提案した。Krishnakant Singhら~\cite{Singh_2024_CVPR}は、合成データを用いて訓練されたモデルの堅牢性をOOD（Out-Of-Distribution）detectionのタスクにおいて、評価している。
%なし
% 合成データを用いて訓練されたモデルは、特定の条件下では実際のデータを用いたモデルと同等かそれ以上の性能を示すことがあると述べている。

% 本研究では、SIDに対して、実画像のみで学習した基盤モデルであるCLIP、DINOv2と生成画像やLLMの合成データを使用して学習した基盤モデルであるStableRep、SynCLRを使用する。

% \subsection{Foundation Model}

% A Foundation Model refers to a general-purpose AI model pre-trained on a large-scale dataset. These models are typically built using self-supervised learning and exhibit high versatility across a wide range of tasks. Widely utilized in various fields, including natural language processing (NLP), image recognition, and speech recognition, foundation models demonstrate significant adaptability.

% \subsubsection{Transformer and Language Models.}

% In 2017, Vaswani~\etal.~\cite{vaswani2017attention} proposed the Transformer architecture, leading to the emergence of multiple foundation models primarily for language tasks. Devlin~\etal~\cite{devlin2018bert} introduced BERT (Bidirectional Encoder Representations from Transformers), a bidirectional Transformer encoder that achieved state-of-the-art results in NLP tasks. Radford\etal~\cite{radford2018improving} proposed GPT, a powerful model for generative tasks utilizing a unidirectional Transformer decoder. Subsequently, Brown\etal~\cite{brown2020language} demonstrated GPT-3's ability to handle a wide range of NLP tasks with a few task examples. Additionally, the T5 (Text-To-Text Transfer Transformer)~\cite{raffel2020exploring} model was introduced, treating all NLP tasks as text generation problems. This approach enhanced the efficiency of transfer learning across tasks by processing various NLP tasks in a unified text generation format.

% \subsubsection{Vision Transformer and Visual Foundation Models.}

% Vision Transformer (ViT)~\cite{dosovitskiy2020image} applied the Transformer architecture to image recognition tasks for the first time, demonstrating high performance without relying on traditional CNNs. This breakthrough led to the emergence of various foundation models. CLIP (Contrastive Language-Image Pre-Training)~\cite{radford2021learning} achieved high performance in visual tasks through pre-training on text-image pairs. DINO (Distillation with NO labels)~\cite{caron2021emerging} is a self-supervised learning method leveraging knowledge distillation to learn feature representations from unlabeled data. An improvement on DINO, DINOv2 (Self-Distillation with No Labels)~\cite{oquab2023dinov2}, extracts high-quality visual features independently of the dataset by combining self-distillation and contrastive learning, achieving superior performance.

% Additionally, MERU~\cite{desai2023meru}, which learns image and language representations in hyperbolic space, effectively captures hierarchical data structures compared to traditional Euclidean space. This approach naturally grasps the relationship between images and language, achieving high accuracy, particularly in image caption generation and image retrieval.

% \subsubsection{Training with Synthetic Images and LLMs.}

% While previous methods focused on learning using real images and text data, training with synthetic images and LLMs has become increasingly common. VisualAtom~\cite{takashima2023visual}, specialized in representation learning of visual data, developed a novel approach based on toroidal harmonics to optimize parameters, leveraging the effectiveness of Formula-driven supervised learning (FDSL) during ViT pre-training. This study confirmed the importance of diversity in synthetic images.

% Tian~\etal proposed Stablerep~\cite{NEURIPS2023_971f1e59}, which conducts self-supervised learning using text data and image generation models without using any real data. They also introduced SynCLR~\cite{Tian_2024_CVPR}, a method for contrastive learning that employs LLMs and image generation models. Krishnakant Singh~\etal ~\cite{Singh_2024_CVPR} evaluated the robustness of models trained with synthetic data in the task of out-of-distribution (OOD) detection.

% \subsubsection{Models Used in This Study.}

% This study employs CLIP and DINOv2, foundational models trained solely on real images, as well as StableRep and SynCLR, foundational models trained using synthetic data from synthetic images and LLMs, for SID.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%memo

% Transformer:Vaswani et al., 2017: Transformerアーキテクチャの提案~\cite{vaswani2017attention}

% BERT (Bidirectional Encoder Representations from Transformers):~\cite{devlin2018bert}
% Devlin et al., 2018: BERTは双方向のTransformerエンコーダを使用し、NLPタスクで最先端の成果を達成した言語表現モデル。


% GPT (Generative Pre-trained Transformer):Radford et al., 2018: GPTは一方向のTransformerデコーダを使用し、生成タスクで強力な性能を示しました。
% Brown et al., 2020: GPT-3は少量のタスク例で幅広いNLPタスクをこなせる能力を示しました。


% T5 (Text-To-Text Transfer Transformer):Raffel et al., 2020: すべてのNLPタスクをテキスト生成問題として扱う。様々なNLPタスクを統一されたテキスト生成形式で処理することで、タスク間の転移学習の効率を向上させる ~\cite{raffel2020exploring}

% Vitが提案された
% Alexey Dosovitskiyらによって提案され、2020年に発表されました。このモデルは、画像認識タスクにおいてTransformerアーキテクチャを初めて適用し、従来のCNNに依存しないアプローチで高い性能を示しました ~\cite{dosovitskiy2020image}

% CLIP (Contrastive Language-Image Pre-Training):Radford et al., 2021: テキストと画像のペアを用いた事前学習で視覚タスクに高い性能を示しました。 ~\cite{radford2021learning}

% DINO：2021 わからん ~\cite{caron2021emerging}

% DINOv2 (Self-Distillation with No Labels):Maxime Oquab., 2023: ラベルなしで頑健な視覚特徴を学習する手法であるDINOv2が提案されています。この手法は、自己教師あり学習を活用し、データセットに依存せずに高品質な視覚特徴を抽出します。DINOv2は従来のDINOを改良し、自己蒸留とコントラスト学習を組み合わせることで、監督なしで優れた性能を達成しています ~\cite{oquab2023dinov2}

% MERU:Karan Desai, 2023: 画像と言語の表現を双曲空間で学習する方法を提案しています。従来のユークリッド空間に比べ、双曲空間は階層的なデータ構造を効果的に表現できるため、画像と言語の関連性をより自然に捉えられます。特に画像キャプション生成や画像検索において高い精度を達成しました。 ~\cite{desai2023meru}

% VisualAtom: Sora Takashima., 2023: ビジュアルデータの表現学習に特化したモデル。ViTの事前学習において、Formula-driven supervised learning（FDSL）が有効であることが示されています。FDSLのパラメータを最適化するために円環調和に基づく新しい手法を開発し、合成画像の多様性が重要であることを確認しました。 ~\cite{takashima2023visual}

% SynCLR (Synchronized Contrastive Learning): Yonglong Tian 2023: マルチモーダルデータのコントラスト学習を同期させる。LLMと画像生成モデルを使用してVitの学習を行った。 ~\cite{tian2023learningvisionmodelsrivals}

% Stablerep: Yonglong Tian 2024?: テキストデータと画像生成モデルを使用してVitの学習を行った ~\cite{tian2024stablerep}

% SynCLR (Synchronized Contrastive Learning): Yonglong Tian 2024: マルチモーダルデータのコントラスト学習を同期させる。LLMと画像生成モデルを使用してVitの学習を行った。SynCLRは合成データを利用してコントラスト学習を行う手法で、自己教師あり学習の一種です。この手法は、データ収集やラベリングのコストを削減し、データの多様性を確保するために合成データを活用します。
% ~\cite{Tian_2024_CVPR}

% Stablerep: Yonglong Tian 2023: テキストデータと画像生成モデルを使用してVitの学習を行った。StableRepは、安定した特徴表現を学習することを目的とした手法で、特に生成モデルや高変動データに対してロバストな表現を提供します。
% ~\cite{NEURIPS2023_971f1e59}


